A Token-level Reference-free Hallucination Detection Benchmark for Free-form Text Generation

Large pretrained generative models like GPT-3 often suffer from hallucinating non-existent or incorrect content, which undermines their potential merits in real applications. Existing work usually attempts to detect these hallucinations based on a corresponding oracle reference at a sentence or document level. However ground-truth references may not be readily available for many free-form text generation applications, and sentence- or document-level detection may fail to provide the fine-grained signals that would prevent fallacious content in real time. As a first step to addressing these issues, we propose a novel token-level, reference-free hallucination detection task and an associated annotated dataset named HaDes (HAllucination DEtection dataSet). To create this dataset, we first perturb a large number of text segments extracted from English language Wikipedia, and then verify these with crowd-sourced annotations. To mitigate label imbalance during annotation, we utilize an iterative model-in-loop strategy. We conduct comprehensive data analyses and create multiple baseline models.

==> pics/introduction_backup.tex <==
\section{Introduction}
% \tianyu{please feel free to make comments}
% \yz{a test}
% \yi{a test}
% \chris{a test}
\yz{in the title, do you want to focus more on task, or the dataset? if it's the latter, maybe change the title to `**** dataset'}
 Automatic text generation using neural natural language generation (NLG) systems is increasingly fluent and thus seemingly plausible in many real-world applications. Large-scale pretrained models like GPT-3 \yz{cite} have been proved to be powerful in understanding and performing many generation tasks at human-quality level with few in-context examples, which dramatically reduces the needed manual labors of many text-based applications and services. 
Nevertheless, despite the great success, machine generated text may not always be trustworthy: neural NLG systems using very large pre-trained models struggle to generate factually accurate text \cite{radford2019language,brown2020language} and exhibit a propensity to hallucinate non-existent or incorrect content that is unacceptable in most user-oriented applications. This poses a major challenge for deploying NLG system with realtime generation, where post-examination is impossible. 

Hallucinations are commonly observed in abstractive summarization \cite{maynez-etal-2020-faithfulness}, machine translation \cite{wang-sennrich-2020-exposure}, data-to-text generation \cite{rebuffel2021controlling}, and image caption generation \cite{rohrbach-etal-2018-object}. 
These existing works focused on \emph{reference-based hallucination detection}, which identifies hallucinated content and quantitatively measures generation consistency against a provided reference. However, for many text generation tasks, 
% (\textit{e.g.} prose/story generation) 
references are not readily available. 
% These include many real-time NLG applications, such as
For example, runtime response generation from a social chatbot, or auto-completion for document.


Another common setup for qualitatively measuring the level of hallucination in the existing literature is that the detection is usually performed at \textit{sentence- or document-level}\cite{dhingra-etal-2019-handling,scialom2019answers}. Related to the hallucination detection, fake news detection \cite{zellers2019neuralfakenews} or fact checking \cite{thorne-vlachos-2018-automated} tasks also adopt such setup. 
However, from a pragmatic point of view, sentence- or document-level hallucination detection may not always provide high-resolution signals to pinpoint the hallucinated text, thus further rendering mitigating the identified hallucination issue difficult.



% , where references are either non-existent or unavailable in real-time.
With such observations, in this work, we propose a \emph{reference-free and token-level hallucination detection} task and annotated training and benchmark test datasets associated with it \yz{detection or risk detection? Either is fine, but need to be consistent}. We hope the proposed task and datasets can facilitate the evaluation and development of identifying fallacious content in machine generated text without requiring reference data. The \textit{reference-free} property of this task yields more flexibility to a broad range of generation applications. The \emph{token-level} property of this task encourages developing models that can detect fine-grained signals of potential hallucination. Such fine-grained signals if can be detected may further enable hallucination mitigation of  NLG systems in realtime.
Solving the task may require not only looking up the context to find self-contradictory statement, but sometimes also resorting to commonsense and world knowledge.

% We aim at recognizing the possibility (risk) of being hallucinations for words in the given context, rather than making a definitive judgement on the factuality of the generated text, like fact checking \cite{thorne-vlachos-2018-automated} or fake news detection \cite{zellers2019neuralfakenews}, given the fact that we have no access to the reference or background knowledge. 

%Although challenging, the task is doable given powerful pretrained models, which are equipped with commonsense reasoning and world knowledge.


\chris{I think most readers will stop at this point and say, wait, isn't the problem that pretrained models are the source of hallucination?}\yz{I totally agree. May still need some work regarding Chris's concern.}

%Specifically we name the task \textbf{hallucination risk detection} to distinguish from fake news detection \cite{zellers2019neuralfakenews} or fact checking \cite{thorne-vlachos-2018-automated} tasks as we are unable to make a definitive claim on the factuality of the generated text without reference and background knowledge, instead we aim at recognizing the possibility (risk) of being hallucinations for specific words in the given context.
%\yz{I changed above towards describing the task rather than the method} %Similar to language model, the hallucination detection model trained in the \emph{reference-free} framework could be used in both reference-based (conditional) and reference-free (unconditional) generation.\yz{I don't understand this sentence}
% \yz{extend the paper regarding why reference-free is important, why it is doable given the powerful pretrained models, which is equipped with commonsense and world knowledge. May need to give some examples. }
% \tianyu{done}

% In order to qualitatively measure the level of hallucination, researchers have proposed \textit{sentence or document-level} evaluation metrics for NLG systems \cite{dhingra-etal-2019-handling,scialom2019answers}. However from a pragmatic point of view, sentence- or document- level hallucination detection can not provide actionable insights on how to modify or mitigate the recognized hallucination,
% instead we perform \emph{word-level hallucination detection} for machine generated text, which can serve as the fine-grained signals for both hallucination prevention in the newly deployed NLG systems, and error correction for the running NLG applications.
%i.e. recognizing the specific words or phrases which are likely to be hallucinations. 
%we name the task \textbf{hallucination risk detection} to distinguish from fake news detection \cite{zellers2019neuralfakenews} or fact checking \cite{thorne-vlachos-2018-automated} tasks as we are unable to make a definitive claim on the factuality of the generated text without reference and background knowledge, instead we aim at recognizing the possibility (risk) of being hallucinations for specific words in the given context.
% \yz{the logic in this paragraph may need some work. maybe first focus on ``reference-free'', then move to ``token-level'' }
% \yz{maybe use another paragraph to talk about token-level detection. Why we need to do token-level detection}
% \tianyu{done}


% Formally we name the proposed word-level reference-free hallucination detection task as \textbf{hallucination risk detection}. We aim at recognizing the possibility (risk) of being hallucinations for words in the given context, rather than making a definitive judgement on the factuality of the generated text, like fact checking \cite{thorne-vlachos-2018-automated} or fake news detection \cite{zellers2019neuralfakenews}, given the fact that we have no access to the reference or background knowledge. 

% As there is no benchmark for hallucination risk detection in the prior work, we

The dataset we created for this task is called \textbf{HA}llucination \textbf{DE}tection data\textbf{S}et (\textsc{Hades}). \yz{I change all Hades to hades}
To create hallucinated text, we corrupt raw text from web using \st{a contextualized pretrained model} BERT model\yz{cite}, with three operations: \textsc{MASK}, \textsc{REPLACE} and \textsc{RANK}. 
% We also set up two different subtask settings, which we call `static' and `dynamic' settings which recognize hallucination in the already generated text, and on-the-fly generation respectively.
%\yz{I comment out above, as they are more related to the detection side of this work}
We further ask human annotators to judge on whether the corrupted text introduces hallucinated contents given the original text.
%\yz{what is a more `robust/generalizable' dataset? Let's discuss} 
We further adopt an adversarial model-in-the-loop strategy \cite{jia-liang-2017-adversarial,zellers-etal-2018-swag,nie-etal-2020-adversarial} to mitigate the label imbalance issue. Several baselines using various  strategies based on manual features and transformer-based models were developed as the initial step towards investigating this problem. 
The boundary between hallucination and factuality is not always clear. We conduct further analysis on \textsc{Hades}, to shed light upon what is commonly recognized as hallucination and their salient characteristics in the machine generated text according to crowd-sourced judgements.




% One challenge of creating such an annotated dataset is that the label imbalance issue, where most of the text tweaked by a pretrained model become ``hallucinated'' to the original text.
% In order to mitigate the annotation artifacts \cite{gururangan-etal-2018-annotation} in the dataset construction, we adopt an adversarial model-in-the-loop strategy \cite{jia-liang-2017-adversarial,zellers-etal-2018-swag,nie-etal-2020-adversarial} to overcome the label imbalance issue. Specifically we train a detection model in an iterative manner, and set up thresholds to select low-confidence ``hallucination'' cases which would be sent to annotators, as excessively high-confidence cases tend to fall into similar linguistic patterns thus too trivial. 

% Besides we observe an extreme imbalanced label distribution, i.e. `hallucination' cases dominate, in the early rounds of annotation, we thus adopt a statistical modification method which filters some potential `hallucination' cases according to detection model predictions and thus leads to a more balanced label distribution. 
%\yz{combined above to make it more concise}

%To achieve high accuracy on \textsc{Hades}, the detection model should be highly contextualized which is capable of identifying 


% From such case studies, we observe that hallucinated content has certain salient characteristics, which accords with human cognition and to some extent explain why hallucination happens. 

% , e.g. irrelevant name entities which diverges from the specific topic(s) in a document are more likely to be misinformation or hallucination, and word spans with higher level of specificity have higher risk to be hallucination
% \yz{comment out the details}

%In this work, we aim at identifying the risk of being hallucination for individual words and phrases in machine generated text. \textbf{Hallucinated content may have certain characteristics compared with factual descriptions}, e.g. specificity [explanation], the relevance with the surrounding context. Given the context, the irrelevant name entities which diverges from the specific topic(s) in a document are more likely to be misinformation or hallucinations. We hope the contextualized models would be able to learn those implicit features for word-level hallucination detection.We thus propose a \textbf{unified task agnostic framework} to detect the hallucinations in the machine generated text.


%Many prior work measure generation fidelity in the document level. In this way, many document level automatic evaluation metrics involving question answering \cite{scialom2019answers,eyal2019question,wang2020asking}, natural language inference \cite{kryscinski2019evaluating,falke2019ranking} and information extraction \cite{zhang2019optimizing,goodrich2019assessing} are 

%\yz{discuss about previous reference-based hallucination detection. introduce our reference-free detection. what's unique for our task and why this is useful, i.e. why reference-free token-level detection is needed. i think we can say sth like for most of the generative LM, references are not available}



%\yz{say sth about contextualized hallucination detection}

%We proposed a hallucination detection dataset named \textsc{Wiki-HaDe}. \textsc{Wiki-HaDe} is proposed as a benchmark dataset for the measurement of word-level hallucination risk for the machine generated text. We collect open-domain raw text from Wikipedia, then replace words or phrases in the raw text with out-of-box pretrained models, finally we ask human annotators to judge whether the replacement is consistent or hallucinated compared with the raw text. The data input is the replaced text with a position tuple that points to the replacement, and the corresponding target label is \textbf{H}allucination or \textbf{C}onsistent.

We summarize our contributions as follows:

(1) We first propose a \textit{reference-free} and \textit{token-level} hallucination detection task, and create an associated \textsc{Hades} dataset with ~11k instances by using an iterative data collection strategy. \yz{i don't see why this is adversarial}
% This is the first \textit{reference-free} and \textit{token-level} hallucination detection benchmark dataset. 
% \chris{If we are going to post this on arXiv, shouldn't we be releasing the dataset at the same time? This will need to go through our dataset release tracker. And if we do so, this may affect double blind submission. }

(2) We create multiple baseline detection models as a first step towards addressing the hallucination problem.

% (3) We adopt an adversarial model-in-the-loop strategy in the human annotation to mitigate label imbalance problem with a statistical rectification method.

(3) We investigate the decision boundary of hallucination in machine generated text through crowd-sourcing and contextualized detection models.

%\yz{The text reads well. Thanks Tianyu. I have some comments: 1. maybe mentioning about the annotated training set in the contribution? 2. About hallucination "risk", I feel it's hard to distinguish if we are predicting the "risk" of hallucination or detecting the hallucination itself. Maybe we just keep the story simpler by saying this is still detecting the hallucination, but later we can explain in the analysis/experiments that the identified hallucinations are associated with certain pattern? 3. In the introduction maybe we still focus on how do people/we define hallucination, why it's so important, what has been done to detect hallucination and what needs to be done?4. Maybe mentioning about hallucination is hard to define, and we are collecting human annotations to help define the problem via crowd-sourcing? Shall we consider this as one contribution?}
\yz{this intro is still a bit long.}
